MADField: Multi-fidelity Amortized Density Field for Adsorption in Nanoporous Materials

High-throughput computational screening of nanoporous materials for gas storage and separation requires fast and accurate characterization of adsorption equilibrium. Particle-based grand canonical Monte Carlo (GCMC) and density-based classical density functional theory (cDFT) provide simulation-based estimates of gas uptake and adsorbate density fields, but their speed-accuracy tradeoff remains insufficient for large-scale screening. In this work, we address this gap with Multi-fidelity Amortized Density Field for Adsorption in Nanoporous Materials (MADField), which reframes adsorption prediction as equilibrium density-field estimation. MADField learns from two complementary fidelities, combining broad and scalable cDFT density supervision with higher-fidelity GCMC density labels, and recovers gas uptake by integrating the predicted density field. MADField improves uptake accuracy over the strongest baselines by 6.0x for cDFT and 15.4x for GCMC, and its predicted fields accelerate cDFT solvers with 2.0x fewer iteration steps while recovering 42 percent of cases that fail under standard settings. Finally, we evaluate MADField for conventional CH4 working capacity screening on the 270k-structure ARC-MOF database. Within this space of extremely rare high-capacity targets, 167 in total, the model achieves 56x higher average precision than the strongest baseline and accelerates inference by five orders of magnitude compared to GCMC. By prioritizing the MADField rankings, selecting the top 1.7 percent of candidates recovers 95 percent of all targets, while the top 6 percent ensures 100 percent recall.

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}



\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    \item[] Justification: The abstract and introduction state the paper's scope as physically scaled, unnormalized 3D adsorbate density prediction for porous materials, with cDFT pretraining, GCMC adaptation, uptake recovery by integration, and cDFT warm-starting.

    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper includes a limitations discussion in the Conclusion section, while we think inherit approximation error of free energy functional, and multi component system as a limitation. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper does not present new theoretical theorems or formal proofs. The mathematical expressions define the adsorption observables, GCMC and cDFT density targets, Boltzmann reference density, Picard fixed-point map, and training losses.
    Their assumptions and derivations are provided as background and implementation definitions rather than as novel theoretical results.

    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper specifies the datasets, fidelity targets, train/validation/test split protocol, model architecture, conditioning variables, loss components, training stages, LoRA adaptation setup, baseline adaptations, evaluation metrics, and inference-time protocol.
    The appendix provides additional details on cDFT/GCMC definitions, data generation, architecture, training, metrics, baselines, warm-start settings, and reproducibility.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper describes the data sources, preprocessing, model architecture, training objectives, optimizer setup, baseline implementations, and evaluation scripts needed to reproduce the reported results.
    Our code and data will be released for reproduction of our work. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: The experimental setup is described in the main paper and appendix, including dataset sources, adsorbate and pressure grids, target definitions, model inputs, training losses, optimizer settings, LoRA adaptation details, baseline task formulations, and evaluation metrics.
    Hardware and inference timing details are also provided in the appendix.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer:  \answerNo{}
    \item[] Justification: The main experiments report deterministic aggregate metrics on fixed train/validation/test splits rather than repeated runs with error bars.
    We report per-adsorbate, per-material-family, and OOD breakdowns to characterize variability across gases, pressures, and material classes, but we do not claim statistical significance across random seeds.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
        \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper reports the GPU type, training setup, number of GPUs, training stages, inference-time measurements, and evaluation modes.
    The appendix specifies that the main models are trained on H200 GPUs, gives stage-wise training details, and reports wall-clock inference time per sample for MADField and the baselines.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The work conforms to the NeurIPS Code of Ethics.
    It uses simulated porous-material structures and published or generated scientific simulation data, does not involve human subjects, personal data, surveillance, or sensitive attributes, and is intended for scientific modeling of adsorption in materials discovery.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{}
    \item[] Justification: We wrote Broader impacts section at the end of the Appendices. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer:  \answerNA{}
    \item[] Justification: The paper does not release assets with high misuse risk such as pretrained language models, image generators, scraped personal data, or safety-sensitive datasets.
    The released assets are scientific simulation code, trained adsorption-density models, and porous-material simulation data.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}
    \item[] Justification: Existing datasets, software packages, and baseline models are cited in the paper and appendix.
    The paper credits QMOF, ARC-MOF/GCMC density references, PRAM, JLA-Gardner amorphous carbon structures, FeOs, ASE, RASPA, and the scalar and density-field baseline codebases.
    Licensing and usage terms will be documented in the released repository and supplementary material where applicable.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper introduces new trained models, generated cDFT data, which will be released under CC-BY 4.0 . The appendix documents their construction, including simulation definitions, pressure grids, target formats, split protocols, training settings, and evaluation metrics.

    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{}
    \item[] Justification: The work does not involve crowdsourcing or user studies. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}
    \item[] Justification: The work does not involve human subjects, human-derived data, interventions, surveys.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{}
    \item[] Justification: LLMs are not used as a core methodological component of the research. LLM did not define the scientific method, model architecture, data generation protocol, or experimental conclusions.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> figures/fig7.tex <==
% Figure 7 -- per-MOF CH4 working-capacity parity (single combined PDF;
% panel grid, spacing and shared colorbar are all baked in -> renders exactly).
\begin{figure}[p]
    \centering
    \includegraphics[width=\linewidth]{figures/fig7_wc_parity.pdf}
    \caption{\textbf{Per-MOF \ce{CH4} working-capacity (WC) parity on the full ARC-MOF 270k database.}
    Each panel compares predicted WC against the GCMC reference across all $270{,}583$ frameworks; hexbin shading counts frameworks per cell on a shared log scale (right colorbar), the red dashed line is $y=x$, and dotted lines mark the $\mathrm{WC}=200~\mathrm{cm^3/cm^3}$ target threshold (per-panel WC MAE in $\mathrm{cm^3/cm^3}$).
    \method{} aligns tightly with the reference across the full range and resolves the rare high-WC regime, whereas the uptake baselines compress their predictions into a narrow band or miss high-WC frameworks entirely.}
    \label{fig:fig7_wc_parity}
\end{figure}


==> figures/fig8.tex <==
% Figure (screening) -- assembled from legend + 3 panel pieces;
% (a)(b)(c) placed at top-left via overpic; legend kept close to the panels.
\begin{figure}[p]
    \centering
    \includegraphics[width=0.92\linewidth]{figures/fig8_legend.pdf}\\[-3pt]
    \begin{overpic}[width=0.325\linewidth]{figures/fig8a_hist.pdf}\put(1,95){\footnotesize\textbf{(a)}}\end{overpic}\hfill
    \begin{overpic}[width=0.325\linewidth]{figures/fig8b_recall.pdf}\put(1,95){\footnotesize\textbf{(b)}}\end{overpic}\hfill
    \begin{overpic}[width=0.325\linewidth]{figures/fig8c_pareto.pdf}\put(1,95){\footnotesize\textbf{(c)}}\end{overpic}
    \caption{\textbf{Database-scale high-capacity MOF screening} on all $270{,}583$ ARC-MOF frameworks for \ce{CH4} working capacity (WC), with $167$ high-WC targets ($\mathrm{WC}\ge 200~\mathrm{cm^3/cm^3}$, $0.06\%$ of the database).
    \textbf{(a)} Distribution of GCMC WC, with the rare high-WC target regime beyond the dashed threshold.
    \textbf{(b)} True targets retrieved as a function of the number of frameworks screened in predicted-WC order; the dashed \emph{Ideal} curve is the upper bound, and \method{} reaches $95\%$ and $100\%$ recall after screening only $4{,}716$ and $16{,}759$ frameworks ($1.7\%$ and $6.2\%$ of the database).
    \textbf{(c)} Average precision (AP) versus per-MOF inference/simulation time. \method{} attains AP $=0.557$, a $56\times$ improvement over the strongest learned baseline (Uni-MOF, $0.010$), while the cDFT-only ablation reaches $0.068$, all at five orders of magnitude lower per-MOF cost than fully converged GCMC.}
    \label{fig:fig8_wc_screening}
\end{figure}


==> submissions.tex <==

\section{Submission of papers to NeurIPS 2026}


Please read the instructions below carefully and follow them faithfully.


\subsection{Style}


Papers to be submitted to NeurIPS 2026 must be prepared according to the
instructions presented here. Papers may only be up to {\bf nine} pages long, including figures. \textbf{Papers that exceed the page limit will not be reviewed (or in any other way considered) for presentation at the conference.}
Additional pages \emph{containing acknowledgments, references, checklist, and optional technical appendices} do not count as content pages. 


The margins in 2026 are the same as those in previous years.


Authors are required to use the NeurIPS \LaTeX{} style files obtainable at the NeurIPS website as indicated below. Please make sure you use the current files and not previous versions. Tweaking the style files may be grounds for desk rejection.


\subsection{Retrieval of style files}


The style files for NeurIPS and other conference information are available on the website at
\begin{center}
  \url{https://neurips.cc}.
\end{center}
% The file \verb+neurips_2026.pdf+ contains these instructions and illustrates the various formatting requirements your NeurIPS paper must satisfy.


The only supported style file for NeurIPS 2026 is \verb+neurips_2026.sty+, rewritten for \LaTeXe{}. \textbf{Previous style files for \LaTeX{} 2.09,  Microsoft Word, and RTF are no longer supported.}


The \LaTeX{} style file contains three optional arguments: 
\begin{itemize}
\item \verb+final+, which creates a camera-ready copy, 
\item \verb+preprint+, which creates a preprint for submission to, e.g., arXiv, \item \verb+nonatbib+, which will not load the \verb+natbib+ package for you in case of package clash.
\end{itemize}


\paragraph{Preprint option}
If you wish to post a preprint of your work online, e.g., on arXiv, using the NeurIPS style, please use the \verb+preprint+ option. This will create a nonanonymized version of your work with the text ``Preprint. Work in progress.'' in the footer. This version may be distributed as you see fit, as long as you do not say which conference it was submitted to. Please \textbf{do not} use the \verb+final+ option, which should \textbf{only} be used for papers accepted to NeurIPS.


At submission time, please omit the \verb+final+ and \verb+preprint+ options. This will anonymize your submission and add line numbers to aid review. Please do \emph{not} refer to these line numbers in your paper as they will be removed during generation of camera-ready copies.


The file \verb+neurips_2026.tex+ may be used as a ``shell'' for writing your paper. All you have to do is replace the author, title, abstract, and text of the paper with your own.


The formatting instructions contained in these style files are summarized in Sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.


\section{General formatting instructions}
\label{gen_inst}


The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).  Use 10~point
type with a vertical spacing (leading) of 11~points.  Times New Roman is the
preferred typeface throughout, and will be selected for you by default.
Paragraphs are separated by \nicefrac{1}{2}~line space (5.5 points), with no
indentation.


The paper title should be 17~point, initial caps/lower case, bold, centered
between two horizontal rules. The top rule should be 4~points thick and the
bottom rule should be 1~point thick. Allow \nicefrac{1}{4}~inch space above and
below the title to rules. All pages should start at 1~inch (6~picas) from the
top of the page.


For the final version, authors' names are set in boldface, and each name is
centered above the corresponding address. The lead author's name is to be listed
first (left-most), and the co-authors' names (if different address) are set to
follow. If there is only one co-author, list both author and co-author side by
side.


Please pay special attention to the instructions in Section \ref{others}
regarding figures, tables, acknowledgments, and references.

\section{Headings: first level}
\label{headings}


All headings should be lower case (except for first word and proper nouns),
flush left, and bold.


First-level headings should be in 12-point type.


\subsection{Headings: second level}


Second-level headings should be in 10-point type.


\subsubsection{Headings: third level}


Third-level headings should be in 10-point type.


\paragraph{Paragraphs}


There is also a \verb+\paragraph+ command available, which sets the heading in
bold, flush left, and inline with the text, with the heading followed by 1\,em
of space.


\section{Citations, figures, tables, references}
\label{others}


These instructions apply to everyone.


\subsection{Citations within the text}


The \verb+natbib+ package will be loaded for you by default.  Citations may be
author/year or numeric, as long as you maintain internal consistency.  As to the
format of the references themselves, any style is acceptable as long as it is
used consistently.


The documentation for \verb+natbib+ may be found at
\begin{center}
  \url{http://mirrors.ctan.org/macros/latex/contrib/natbib/natnotes.pdf}
\end{center}
Of note is the command \verb+\citet+, which produces citations appropriate for
use in inline text.  For example,
\begin{verbatim}
   \citet{hasselmo} investigated\dots
\end{verbatim}
produces
\begin{quote}
  Hasselmo, et al.\ (1995) investigated\dots
\end{quote}


If you wish to load the \verb+natbib+ package with options, you may add the
following before loading the \verb+neurips_2026+ package:
\begin{verbatim}
   \PassOptionsToPackage{options}{natbib}
\end{verbatim}


If \verb+natbib+ clashes with another package you load, you can add the optional
argument \verb+nonatbib+ when loading the style file:
\begin{verbatim}
   \usepackage[nonatbib]{neurips_2026}
\end{verbatim}


As submission is double blind, refer to your own published work in the third
person. That is, use ``In the previous work of Jones et al.\ [4],'' not ``In our
previous work [4].'' If you cite your other papers that are not widely available
(e.g., a journal paper under review), use anonymous author names in the
citation, e.g., an author of the form ``A.\ Anonymous'' and include a copy of the anonymized paper in the supplementary material.


\subsection{Footnotes}


Footnotes should be used sparingly.  If you do require a footnote, indicate
footnotes with a number\footnote{Sample of the first footnote.} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches (12~picas).


Note that footnotes are properly typeset \emph{after} punctuation
marks.\footnote{As in this example.}


\subsection{Figures}


\begin{figure}
  \centering
  \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \caption{Sample figure caption. Explain what the figure shows and add a key take-away message to the caption.}
\end{figure}


All artwork must be neat, clean, and legible. Lines should be dark enough for
 reproduction purposes. The figure number and caption always appear after the
figure. Place one line space before the figure caption and one line space after
the figure. The figure caption should be lower case (except for the first word and proper nouns); figures are numbered consecutively.


You may use color figures.  However, it is best for the figure captions and the
paper body to be legible if the paper is printed in either black/white or in
color.


\subsection{Tables}


All tables must be centered, neat, clean, and legible.  The table number and
title always appear before the table.  See Table~\ref{sample-table}.


Place one line space before the table title, one line space after the
table title, and one line space after the table. The table title must
be lower case (except for the first word and proper nouns); tables are
numbered consecutively.


Note that publication-quality tables \emph{do not contain vertical rules}. We
strongly suggest the use of the \verb+booktabs+ package, which allows for
typesetting high-quality, professional tables:
\begin{center}
  \url{https://www.ctan.org/pkg/booktabs}
\end{center}
This package was used to typeset Table~\ref{sample-table}.


\begin{table}
  \caption{Sample table caption. Explain what the table shows and add a key take-away message to the caption.}
  \label{sample-table}
  \centering
  \begin{tabular}{lll}
    \toprule
    \multicolumn{2}{c}{Part}                   \\
    \cmidrule(r){1-2}
    Name     & Description     & Size ($\mu$m) \\
    \midrule
    Dendrite & Input terminal  & $\approx$100     \\
    Axon     & Output terminal & $\approx$10      \\
    Soma     & Cell body       & up to $10^6$  \\
    \bottomrule
  \end{tabular}
\end{table}

\subsection{Math}
Note that display math in bare TeX commands will not create correct line numbers for submission. Please use LaTeX (or AMSTeX) commands for unnumbered display math. (You really shouldn't be using \$\$ anyway; see \url{https://tex.stackexchange.com/questions/503/why-is-preferable-to} and \url{https://tex.stackexchange.com/questions/40492/what-are-the-differences-between-align-equation-and-displaymath} for more information.)

\subsection{Final instructions}

Do not change any aspects of the formatting parameters in the style files.  In
particular, do not modify the width or length of the rectangle the text should
fit into, and do not change font sizes. Please note that pages should be
numbered.


\section{Preparing PDF files}


Please prepare submission files with paper size ``US Letter,'' and not, for
example, ``A4.''


Fonts were the main cause of problems in the past years. Your PDF file must only
contain Type 1 or Embedded TrueType fonts. Here are a few instructions to
achieve this.


\begin{itemize}


\item You should directly generate PDF files using \verb+pdflatex+.


\item You can check which fonts a PDF files uses.  In Acrobat Reader, select the
  menu Files$>$Document Properties$>$Fonts and select Show All Fonts. You can
  also use the program \verb+pdffonts+ which comes with \verb+xpdf+ and is
  available out-of-the-box on most Linux machines.


\item \verb+xfig+ ``patterned'' shapes are implemented with bitmap fonts.  Use
  "solid" shapes instead.


\item The \verb+\bbold+ package almost always uses bitmap fonts.  You should use
  the equivalent AMS Fonts:
\begin{verbatim}
   \usepackage{amsfonts}
\end{verbatim}
followed by, e.g., \verb+\mathbb{R}+, \verb+\mathbb{N}+, or \verb+\mathbb{C}+
for $\mathbb{R}$, $\mathbb{N}$ or $\mathbb{C}$.  You can also use the following
workaround for reals, natural and complex:
\begin{verbatim}
   \newcommand{\RR}{I\!\!R} %real numbers
   \newcommand{\Nat}{I\!\!N} %natural numbers
   \newcommand{\CC}{I\!\!\!\!C} %complex numbers
\end{verbatim}
Note that \verb+amsfonts+ is automatically loaded by the \verb+amssymb+ package.


\end{itemize}


If your file contains type 3 fonts or non embedded TrueType fonts, we will ask
you to fix it.


\subsection{Margins in \LaTeX{}}


Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+ from the \verb+graphicx+ package. Always specify the
figure width as a multiple of the line width as in the example below:
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
See Section 4.4 in the graphics bundle documentation
(\url{http://mirrors.ctan.org/macros/latex/required/graphics/grfguide.pdf})


A number of width problems arise when \LaTeX{} cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command when
necessary.

\begin{ack}
Use unnumbered first level headings for the acknowledgments. All acknowledgments
go at the end of the paper before the list of references. Moreover, you are required to declare
funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work).
More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2026/PaperInformation/FundingDisclosure}.


Do {\bf not} include this section in the anonymized submission, only in the final paper. You can use the \texttt{ack} environment provided in the style file to automatically hide this section in the anonymized submission.
\end{ack}

\section*{References}


References follow the acknowledgments in the camera-ready paper. Use unnumbered first-level heading for
the references. Any choice of citation style is acceptable as long as you are
consistent. It is permissible to reduce the font size to \verb+small+ (9 point)
when listing the references.
Note that the Reference section does not count towards the page limit.
\medskip


{
\small


[1] Alexander, J.A.\ \& Mozer, M.C.\ (1995) Template-based algorithms for
connectionist rule extraction. In G.\ Tesauro, D.S.\ Touretzky and T.K.\ Leen
(eds.), {\it Advances in Neural Information Processing Systems 7},
pp.\ 609--616. Cambridge, MA: MIT Press.


[2] Bower, J.M.\ \& Beeman, D.\ (1995) {\it The Book of GENESIS: Exploring
  Realistic Neural Models with the GEneral NEural SImulation System.}  New York:
TELOS/Springer--Verlag.


[3] Hasselmo, M.E., Schnell, E.\ \& Barkai, E.\ (1995) Dynamics of learning and
recall at excitatory recurrent synapses and cholinergic modulation in rat
hippocampal region CA3. {\it Journal of Neuroscience} {\bf 15}(7):5249-5262.
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\appendix

\section{Technical appendices and supplementary material}
Technical appendices with additional results, figures, graphs, and proofs may be submitted with the paper submission before the full submission deadline (see above). You can upload a ZIP file for videos or code, but do not upload a separate PDF file for the appendix. There is no page limit for the technical appendices. 

Note: Think of the appendix as ``optional reading'' for reviewers. The paper must be able to stand alone without the appendix; for example, adding critical experiments that support the main claims to an appendix is inappropriate. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newpage
\input{checklist.tex}

==> tables/GCMC_density.tex <==
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.15}
\begin{table}[t]
\caption{\textbf{GCMC density prediction quality.}
Tanimoto similarity ($\uparrow$) measures the overlap between predicted and reference normalized density fields on the same GCMC split.
DeepAPD and SorbIIT predict normalized density fields, while UniRho-GCMC predicts absolute density and is normalized only for this shape-similarity evaluation.
}
\label{tab:gcmc_density}
\footnotesize
\centering
\begin{tabular}{l ccc}
\toprule
\multirow{2}{*}{Model}
 & \multicolumn{3}{c}{Tanimoto similarity ($\uparrow$).} \\
\cmidrule(l){2-4}
 & \ce{CH4} & \ce{Xe} & \textbf{Total} \\
\midrule
SorbIIT
 & 0.730 & 0.690 & 0.717 \\
DeepAPD
 & 0.904 & 0.863 & 0.891 \\
UniRho-GCMC (scratch)
 & 0.969 & 0.912 & 0.950 \\
\textbf{UniRho-GCMC}
 & \textbf{0.982} & \textbf{0.931} & \textbf{0.965} \\
\bottomrule
\end{tabular}
\end{table}

% \setlength{\tabcolsep}{6pt}
% \renewcommand{\arraystretch}{1.15}
% \begin{table}[t]
% \caption{\textbf{GCMC density prediction quality.}
% Tanimoto similarity ($\uparrow$) measures the overlap between predicted and reference normalized density fields on the same GCMC split.
% DeepAPD and SorbIIT predict normalized density fields, while UniRho-GCMC predicts absolute density and is normalized only for this shape-similarity evaluation.
% }
% \label{tab:gcmc_density}
% \footnotesize
% \centering
% \begin{tabular}{l ccc}
% \toprule
% \multirow{2}{*}{Model}
%  & \multicolumn{3}{c}{Tanimoto similarity ($\uparrow$).} \\
% \cmidrule(l){2-4}
%  & \ce{CH4} & \ce{Xe} & \textbf{Total} \\
% \midrule
% SorbIIT
%  & 0.73 & 0.69 & 0.717 \\
% DeepAPD
%  & 0.9043 & 0.863 & 0.891 \\
% UniRho-GCMC (scratch)
%  & 0.969 & 0.912 & 0.950 \\
% \textbf{UniRho-GCMC}
%  & \textbf{\ptz0.9823} & \textbf{0.9307} & \textbf{0.9651} \\
% \bottomrule
% \end{tabular}
% \end{table}

==> tables/GCMC_uptake.tex <==
\setlength{\tabcolsep}{5.5pt}
\renewcommand{\arraystretch}{1.18}

\begin{table}[t]
\caption{\textbf{GCMC gas uptake prediction with PRAM zero-shot transfer.}
Errors are MAE of gas uptake in cm$^3$(STP)/g, except PRAM MRE, reported in \%.
\textbf{MOF (ID)}: in-distribution evaluation on crystalline MOFs.
\textbf{PRAM (OOD)}: zero-shot transfer to amorphous nanoporous materials (\ce{CH4} only)
across four material families, with \textbf{Tot.} the sample-weighted mean across families.
Models marked with $^{\dagger}$ predict the full 3D density field.
UniRho-GCMC (scratch) is an ablation trained directly on the GCMC split without cDFT pretraining.
UniRho-GCMC is the cDFT-pretrained, LoRA fine-tuned variant.
\emph{Right panel}: representative PRAM structures used as illustrative examples ---
\emph{top}: PIM-Colina-id001 from the PIM class, 
\emph{bottom}: aCarbon-Bhatia-id001 from the Bhatia class.}
\label{tab:gcmc_uptake}
\centering
\vspace{3pt}

\newsavebox{\tabbox}
\sbox{\tabbox}{\footnotesize
\begin{tabular}{@{}l ccc cccccc@{}}
\toprule
\multirow{2}{*}{Model}
& \multicolumn{3}{c}{MOF (ID)}
& \multicolumn{6}{c}{PRAM (OOD, \ce{CH4})} \\
\cmidrule(lr){2-4} \cmidrule(l){5-10}
& \ce{CH4} & \ce{Xe} & \textbf{Tot.}
& PIM & HCP & Kerog. & Bhatia & \textbf{Tot.} & MRE (\%) \\
\midrule
\emph{Per-(ads., P)} \\
\ptz\ptz RetNet
& 10.72 & 10.65 & 10.70
& \ptz2.28 & \ptz1.94 & \ptz6.36 & \ptz\ptz9.51 & \ptz2.61 & 16.00 \\
\arrayrulecolor{black!40}\midrule\arrayrulecolor{black}

\emph{Per-adsorbate} \\
\ptz\ptz DeepSorption
& 12.73 & 20.19 & 15.21
& \ptz6.14 & \ptz6.72 & 26.80 & \ptz23.10 & \ptz8.17 & 70.60 \\
\ptz\ptz MOFTransformer
& \ptz7.22 & 12.32 & \ptz9.77
& \ptz6.90 & 13.10 & 13.60 & \ptz30.60 & 10.03 & 69.50 \\
\arrayrulecolor{black!40}\midrule\arrayrulecolor{black}

\emph{Cond-(ads., P)} \\

\ptz\ptz IsothermNet
& 16.26 & 21.78 & 18.10
& \ptz9.63 & 11.41 & 44.23 & \ptz46.03 & 13.48 & 71.58 \\
\ptz\ptz Uni-MOF
& \ptz8.11 & 12.29 & 10.20
& \ptz8.20 & \ptz6.10 & 27.80 & \ptz26.90 & \ptz9.48 & 61.10 \\
\ptz\ptz UniRho-GCMC (scratch)$^{\dagger}$
& \ptz0.89 & \ptz3.14 & \ptz1.68
& 10.06 & 10.39 & 22.35 & 102.65 & 13.60 & 72.01 \\
\ptz\ptz \textbf{UniRho-GCMC}$^{\dagger}$
& \ptz\textbf{0.33} & \ptz\textbf{1.37} & \ptz\textbf{0.58}
& \ptz\textbf{0.56} & \ptz\textbf{0.40} & \ptz\textbf{1.42}
& \ptz\ptz\textbf{7.02} & \ptz\textbf{0.75} & \ptz\textbf{6.50} \\
\bottomrule
\end{tabular}}

\noindent
\begin{minipage}[t]{0.8\textwidth}
\vspace{0pt}
\centering
\resizebox{\linewidth}{!}{\usebox{\tabbox}}
\end{minipage}%
\hfill
\begin{minipage}[t]{0.17\textwidth}
\vspace{0pt}
\centering
\includegraphics[
    width=\linewidth,
    height=0.8\dimexpr\ht\tabbox+\dp\tabbox\relax,
    keepaspectratio
]{figures/figure_vertical_ac.pdf}
\end{minipage}

\end{table}

==> tables/cDFT_ablation.tex <==
% tables/cDFT_ablation.tex
\setlength{\tabcolsep}{4.0pt}
\renewcommand{\arraystretch}{1.15}
\begin{table}[t]
\caption{
\textbf{Architecture ablation on cDFT prediction.}
Each row removes one component from the full UniRho-cDFT and retrains from scratch under matched data, conditioning, and optimizer settings.
$N_{\mathrm{err}}$ is the macro-fluid median uptake error in cm$^3$(STP)/g over the nine-adsorbate held-out QMOF test split.
The density-vs-scalar comparison, the largest single ablation, is reported in \cref{sec:cdft_density_vs_scalar}.
}
\label{tab:cdft_ablation}
\footnotesize
\centering
\begin{tabular}{l c c}
\toprule
Configuration & $N_{\mathrm{err}}$ (cm$^3$(STP)/g) & $\Delta$ vs.\ Full \\
\midrule
\textbf{Full UniRho-cDFT} & $\mathbf{0.82}$ & --- \\
\midrule
$-$ Boltzmann-residual output (direct $\rho$ prediction) & $1.01$ & $+0.19$ \\
$-$ PC-SAFT conditioning (one-hot adsorbate index) & $X.XX$ & $+Y.YY$ \\
$-$ Swin 3D U-Vit backbone (FNO) & $3.66$ & $+2.24$ \\
\bottomrule
\end{tabular}
\end{table}

==> tables/cDFT_density.tex <==
\setlength{\tabcolsep}{4.0pt}
\renewcommand{\arraystretch}{1.15}


\begin{table}[t]
\caption{
\textbf{cDFT density prediction accuracy.}
A single jointly trained model evaluated on held-out test splits.
\emph{Crystalline MOFs (QMOF)}: nine non-polar adsorbates spanning PC-SAFT parameters $m \in [1.0, 2.53]$, $\sigma \in [2.58, 3.93]$\,\AA, $\varepsilon/k_B \in [34, 228]$\,K, with errors as medians over (structure, pressure) pairs.
\emph{Amorphous carbons}: $1{,}092$ disordered structures from~\citet{gardner2023synthetic} on CH$_4$, evaluated zero-shot against cDFT-converged references; ``pred/GT'' is the median ratio of predicted to reference loading.
$W^{\mathrm{val}}$ is the 1D Wasserstein distance between empirical CDFs of log-density values.
}
\label{tab:cdft_results}
\footnotesize
\centering
\begin{tabular}{l l c c c c c c}
\toprule
Material 
  & Species 
  & \# struct.\ 
  & $\rho_{\mathrm{err}}$ (\%) 
  & $N_{\mathrm{err}}$ (\%)
  & $W^{\mathrm{val}}$
  & Pearson $r$
  & Time (s) \\
\midrule
\multirow{10}{*}{MOFs} 
  & H$_2$       & $100$  & $0.26$  & $0.08$ & $0.0006$ & ---    & $0.20$ \\
  & Ar          & $140$  & $0.42$  & $0.11$ & $0.0008$ & ---    & $0.20$ \\
  & Kr          & $61$   & $1.39$  & $0.35$ & $0.0013$ & ---    & $0.20$ \\
  & Xe          & $71$   & $3.95$  & $0.81$ & $0.0035$ & ---    & $0.20$ \\
  & N$_2$       & $226$  & $1.66$  & $0.45$ & $0.0014$ & ---    & $0.20$ \\
  & CH$_4$      & $200$  & $2.54$  & $0.37$ & $0.0018$ & ---    & $0.20$ \\
  & CO$_2$      & $254$  & $4.87$  & $0.68$ & $0.0290$ & ---    & $0.20$ \\
  & C$_2$H$_6$  & $89$   & $4.98$  & $0.65$ & $0.0059$ & ---    & $0.20$ \\
  & C$_3$H$_8$  & $189$  & $8.31$ & $0.60$ & $0.0166$ & ---    & $0.20$ \\
  & \textbf{Macro median} & --- & $\mathbf{3.49}$ & $\mathbf{0.46}$ & $\mathbf{0.0018}$ & --- & $\mathbf{0.20}$ \\
\midrule
Amorphous carbons & CH$_4$ & $1{,}092$ & --- & $3.70$ & --- & $0.99$ & $0.20$ \\
\bottomrule
\end{tabular}
\end{table}

==> tables/cDFT_uptake_and_density.tex <==
\setlength{\tabcolsep}{4.0pt}
\renewcommand{\arraystretch}{1.15}

\begin{table}[t]
\caption{\textbf{cDFT uptake prediction benchmark.}
Gas uptake prediction error is reported as MAE in cm$^3$(STP)/g ($\downarrow$) across nine adsorbates.
All baselines are scalar regressors; $^{\dagger}$ denotes models that predict the full 3D equilibrium density field and obtain uptake by integration.
Models are grouped by training paradigm: \emph{Per-(adsorbate, pressure)} (one model per adsorbate per pressure point), \emph{Per-adsorbate} (one model per adsorbate, all pressures), and \emph{Cond-(adsorbate, pressure)} (single model handles all adsorbates and pressures).
Within each group, models are ordered by macro-mean Total (best first).}
\label{tab:cdft_uptake}
\footnotesize
\centering
\resizebox{1.0\textwidth}{!}{%
\begin{tabular}{l l ccccccccc c c}
\toprule
& \multirow{2}{*}{Model} & \multicolumn{10}{c}{MOF (ID)} & \multicolumn{1}{c}{AC (OOD)} \\
\cmidrule(lr){3-12} \cmidrule(l){13-13}
& & \ce{H2} & \ce{Ar} & \ce{Kr} & \ce{Xe} & \ce{N2} & \ce{CH4} & \ce{CO2} & \ce{C2H6} & \ce{C3H8} & \textbf{Total} & \ce{CH4} \\
\midrule
\emph{Per-(ads., P)} & RetNet
& \ptz4.83 & \ptz3.93 & \ptz9.46 & 22.05 & \ptz3.31 & 17.44 & 17.91 & 27.70 & 46.62 & 17.03 & 21.30 \\
\arrayrulecolor{black!40}\midrule\arrayrulecolor{black}
\multirow{2}{*}{\emph{Per-ads.}}
& DeepSorption
& \ptz4.07 & \ptz5.00 & 10.65 & 21.24 & \ptz3.66 & 12.71 & 21.19 & 19.19 & 45.37 & 15.90 & 52.50 \\
& MOFTransformer
& \ptz0.12 & \ptz1.87 & \ptz6.21 & 15.09 & \ptz1.32 & \ptz5.32 & 12.12 & 15.66 & 23.40 & \ptz9.01 & 56.40 \\
\arrayrulecolor{black!40}\midrule\arrayrulecolor{black}
\multirow{4}{*}{\emph{Cond-(ads., P)}}
& IsothermNet
& \ptz5.21 & \ptz7.53 & 18.71 & 40.25 & \ptz5.53 & 21.71 & 44.11 & 52.15 & 81.59 & 21.79 & 13.33 \\
& Uni-MOF
& \ptz0.46 & \ptz1.81 & \ptz5.11 & 12.21 & \ptz1.22 & \ptz4.13 & 10.39 & 11.81 & 22.12 & \ptz7.70 & 31.30 \\
& UniRho-Scalar
& \ptz2.46 & \ptz2.17 & \ptz4.71 & 11.93 & \ptz1.72 & \ptz9.06 & \ptz8.41 & 10.85 & 17.66 & \ptz5.91 & \ptz5.18 \\
& \textbf{UniRho-cDFT}$^{\dagger}$
& \ptz\textbf{0.08} & \ptz\textbf{0.11} & \ptz\textbf{0.49} & \ptz\textbf{2.87} & \ptz\textbf{0.13} & \ptz\textbf{0.80} & \ptz\textbf{1.17} & \ptz\textbf{2.01} & \ptz\textbf{4.51} & \ptz\textbf{0.82} & \ptz\textbf{2.71} \\
\bottomrule
\end{tabular}
}
\end{table}

\setlength{\tabcolsep}{4.0pt}
\renewcommand{\arraystretch}{1.15}

\begin{table}[t]
\caption{\textbf{cDFT density prediction benchmark.}
Normalized density prediction quality is measured by Tanimoto similarity ($\uparrow$) between predicted and ground-truth normalized density fields, computed voxel-wise on the pore region.
Total is the macro-mean across adsorbates.
Time ($\downarrow$) is per-structure inference cost in seconds, averaged across the test set.
All models marked with $^{\dagger}$ predict full 3D density fields.}
\label{tab:cdft_density}
\footnotesize
\centering
\resizebox{0.88\textwidth}{!}{%
\begin{tabular}{l ccccccccc c c}
\toprule
\multirow{2}{*}{Model} & \multicolumn{10}{c}{MOF (ID)} & {Time (s)} \\
\cmidrule(lr){2-11} \cmidrule(lr){12-12}
 & \ce{H2} & \ce{Ar} & \ce{Kr} & \ce{Xe} & \ce{N2} & \ce{CH4} & \ce{CO2} & \ce{C2H6} & \ce{C3H8} & \textbf{Total} & \\
\midrule
SorbIIT$^{\dagger}$
 & 0.881 & 0.749 & 0.693 & 0.736 & 0.812 & 0.714 & 0.908 & 0.819 & 0.823 & 0.793 & x.xx \\
DeepAPD$^{\dagger}$
& 0.968 & 0.955 & 0.942 & 0.905 & 0.958 & 0.947 & 0.929 & 0.902 & 0.849 & 0.928 & x.xx \\
\textbf{UniRho-cDFT}$^{\dagger}$
& \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{0.978} & \textbf{1.000} & \textbf{0.999} & \textbf{0.998} & \textbf{0.991} & \textbf{0.960} & \textbf{0.992} & \textbf{0.20} \\
\bottomrule
\end{tabular}
}
\end{table}

\iffalse
\setlength{\tabcolsep}{4.0pt}
\renewcommand{\arraystretch}{1.15}
\begin{table}[t]
\caption{\textbf{cDFT prediction benchmarks.}
(a) Gas uptake MAE [cm$^3$(STP)/g] ($\downarrow$) across nine adsorbates.
All baselines are scalar regressors; $^{\dagger}$ denotes models that predict the full 3D equilibrium density field and obtain uptake by integration.
Models are grouped by training paradigm: \emph{Per-(adsorbate, pressure)} (one model per adsorbate per pressure point), \emph{Per-adsorbate} (one model per adsorbate, all pressures), and \emph{Cond-(adsorbate, pressure)} (single model handles all adsorbates and pressures).
Within each group, models are ordered by macro-mean Total (best first).
(b) Normalized density prediction quality measured by Tanimoto similarity ($\uparrow$) between predicted and ground-truth normalized density fields, computed voxel-wise on the pore region.
Total is the macro-mean across adsorbates.
Time ($\downarrow$) is per-structure inference cost in seconds, averaged across the test set.}
\label{tab:cdft_combined}
\footnotesize
\centering

\begin{subtable}{\linewidth}
\caption{Gas uptake MAE [cm$^3$(STP)/g] ($\downarrow$).}
\label{tab:cdft_uptake}
\centering
\resizebox{1.0\textwidth}{!}{%
\begin{tabular}{l l ccccccccc c c}
\toprule
& \multirow{2}{*}{Model} & \multicolumn{10}{c}{MOF (ID)} & \multicolumn{1}{c}{AC (OOD)} \\
\cmidrule(lr){3-12} \cmidrule(l){13-13}
& & \ce{H2} & \ce{Ar} & \ce{Kr} & \ce{Xe} & \ce{N2} & \ce{CH4} & \ce{CO2} & \ce{C2H6} & \ce{C3H8} & \textbf{Total} & \ce{CH4} \\
\midrule
\emph{Per-(ads., P)} & RetNet
& \ptz4.83 & \ptz3.93 & \ptz9.46 & 22.05 & \ptz3.31 & 17.44 & 17.91 & 27.70 & 46.62 & 17.03 & \ptz21.30 \\
\arrayrulecolor{black!40}\midrule\arrayrulecolor{black}
\multirow{2}{*}{\emph{Per-ads.}}
& DeepSorption
& \ptz4.07 & \ptz5.00 & 10.65 & 21.24 & \ptz3.66 & 12.71 & 21.19 & 19.19 & 45.37 & 15.90 & \ptz52.50 \\
& MOFTransformer
& \ptz0.12 & \ptz1.87 & \ptz6.21 & 15.09 & \ptz1.32 & \ptz5.32 & 12.12 & 15.66 & 23.40 & \ptz9.01 & \ptz56.40 \\
\arrayrulecolor{black!40}\midrule\arrayrulecolor{black}
\multirow{4}{*}{\emph{Cond-(ads., P)}}
& IsothermNet
& \ptz5.21 & \ptz7.53 & 18.71 & 40.25 & \ptz5.53 & 21.71 & 44.11 & 52.15 & 81.59 & 21.79 & \ptz13.33 \\
& Uni-MOF
& \ptz0.46 & \ptz1.81 & \ptz5.11 & 12.21 & \ptz1.22 & \ptz4.13 & 10.39 & 11.81 & 22.12 & \ptz7.70 & \ptz31.30 \\
& UniRho-Scalar
& \ptz2.46 & \ptz2.17 & \ptz4.71 & 11.93 & \ptz1.72 & \ptz9.06 & \ptz8.41 & 10.85 & 17.66 & \ptz5.91 & \ptz\ptz5.18 \\
& \textbf{UniRho-cDFT}$^{\dagger}$
& \ptz\textbf{0.08} & \ptz\textbf{0.11} & \ptz\textbf{0.49} & \ptz\textbf{2.87} & \ptz\textbf{0.13} & \ptz\textbf{0.80} & \ptz\textbf{1.17} & \ptz\textbf{2.01} & \ptz\textbf{4.51} & \ptz\textbf{0.82} & \ptz\textbf{2.71} \\
\bottomrule
\end{tabular}
}
\end{subtable}

\vspace{1em}

\begin{subtable}{\linewidth}
\caption{Normalized density Tanimoto similarity ($\uparrow$).}
\label{tab:cdft_density}
\centering
\resizebox{0.88\textwidth}{!}{%
\begin{tabular}{l ccccccccc c c}
\toprule
\multirow{2}{*}{Model} & \multicolumn{10}{c}{MOF (ID)} & {Time (s)} \\
\cmidrule(lr){2-11} \cmidrule(lr){12-12}
 & \ce{H2} & \ce{Ar} & \ce{Kr} & \ce{Xe} & \ce{N2} & \ce{CH4} & \ce{CO2} & \ce{C2H6} & \ce{C3H8} & \textbf{Total} & \\
\midrule
SorbIIT$^{\dagger}$
 & 0.881 & 0.749 & 0.693 & 0.736 & 0.812 & 0.714 & 0.908 & 0.819 & 0.823 & 0.793 & x.xx \\
DeepAPD$^{\dagger}$
& 0.968 & 0.955 & 0.942 & 0.905 & 0.958 & 0.947 & 0.929 & 0.902 & 0.849 & 0.928 & x.xx \\
\textbf{UniRho-cDFT$^{\dagger}$}
& \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{0.978} & \textbf{1.000} & \textbf{0.999} & \textbf{0.998} & \textbf{0.991} & \textbf{0.960} & \textbf{0.992} & \textbf{0.20} \\
\bottomrule
\end{tabular}
}
\end{subtable}
\end{table}
\fi

==> tables/density_transferability.tex <==
\setlength{\tabcolsep}{6.0pt}
\renewcommand{\arraystretch}{1.15}

\begin{table}[t]
\caption{\textbf{Density prediction on .}
Tanimoto similarity ($\uparrow$) measures the overlap between predicted and reference normalized density fields on the same GCMC split.
DeepAPD and SorbIIT predict normalized density fields, while UniRho-GCMC predicts absolute density and is normalized only for this shape-similarity evaluation.
}
\label{tab:gcmc_density}
\footnotesize
\centering
\begin{tabular}{l ccc}
\toprule
\multirow{2}{*}{Model}
 & \multicolumn{3}{c}{Tanimoto similarity ($\uparrow$).} \\
\cmidrule(l){2-4}
 & \ce{CH4} & \ce{Xe} & \textbf{Total} \\
\midrule
SorbIIT
 & 0.730 & 0.690 & 0.717 \\
DeepAPD
 & 0.904 & 0.863 & 0.891 \\
\textbf{MADField-GCMC}
 & \textbf{0.982} & \textbf{0.931} & \textbf{0.965} \\
\bottomrule
\end{tabular}
\end{table}
